A population of transition disks around evolved stars: Fingerprints of planets? Catalog of disks surrounding Galactic post-AGB binaries

Post-asymptotic giant branch (post-AGB) binaries are surrounded by massive disks of gas and dust that are similar to protoplanetary disks around young stars. We assembled a catalog of all known Galactic post-AGB binaries with disks. We explore the correlations between the different observables with the aim of learning more about potential disk-binary interactions. We compiled spectral energy distributions of 85 Galactic post-AGB binary systems. We built a color-color diagram to differentiate between the different disk morphologies traced by the infrared excess. We categorized the different disk types and searched for correlations with other observational characteristics of these systems. Between 8 and 12% of our targets are surrounded by transition disks, that is, disks having no or low near-infrared excess. We find a strong link between these transition disks and the depletion of refractory elements on the surface of the post-AGB star. We interpret this link as evidence of a mechanism that stimulates the dust and gas separation within the disk and that also produces the transition disk structure. We propose that such a mechanism is likely to be due to a giant planet carving a hole in the disk, effectively trapping the dust in the outer disk parts. We propose disk evolutionary scenarios, depending on the presence of such a giant planet in the disk. We advocate that giant planets can successfully explain the link between the transition disks and the observed depletion of refractory materials. If the planetary scenario is confirmed, disks around post-AGB binaries could be a unique laboratory for testing planet-disk interactions and their influence on the late evolution of binary stars. The question of whether such planets are first- or second-generation bodies remains to be considered. We argue that these disks are ideal for studying planet formation in unprecedented parameter space.

==> Fig/TableCat0.tex <==
\begin{table}
	\begin{center}
		\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
			IRAS & Name & RA & DEC & T$_\mathrm{eff}$ (K) & P$_\mathrm{orb}$ (days) & $e$ & H-K$_\mathrm{s}$ & W1-W3 & [Fe/H] & [Zn/Ti] & T$_\mathrm{Turn-off}$ & IR Lum. (\%) & Ref. \\
			\hline
			IRAS06108+2743 & SU Gem  & 06 14 00.0227 & +27 42 12.218 & 5750 & 690 & nan & 1.45$\pm$0.04 & 3.10$\pm$0.08 & -0.700 & 0.500 & 1400 & 310 & - \\
			IRAS06176-1036 & HD_44179 & 06 19 58.2160 & -10 38 14.691 & 7500 & 317.600 & 0.270 & 1.44$\pm$0.25 & 4.48$\pm$0.28 & -3.300 & nan & 1000 & nan & - \\
			IRAS08011-3627 &  AR_Pup  & 08 03 01.1 & -36 35 47 & 6000 & 1250 & nan & 1.51$\pm$0.05 & 3.66$\pm$0.40 & -1 & nan & 1200 & 639 & - \\
			IRAS15556-5444 &  ------  & 15 59 32.1 & -54 53 18 & 6000 & nan & nan & 1.16$\pm$0.04 & 3.94$\pm$0.08 & 0 & nan & nan & 215 & - \\
			IRAS18158-3445 &  ------  & 18 19 13.6 & -34 44 32 & 6500 & nan & nan & 1.27$\pm$0.04 & 3.19$\pm$0.04 & 0 & nan & nan & 126 & - \\
			IRAS19125+0343 & BD+03 3950 & 19 15 01.1809 & +03 48 42.703 & 7750 & 519.700 & 0.240 & 1.29$\pm$0.04 & 3.38$\pm$0.14 & -0.500 & 2.300 & 1400 & 119 & - \\
			IRAS19472+4254 & DF Cyg & 19 48 53.9423 & +43 02 14.529 & 4800 & 784 & nan & 1.16$\pm$0.02 & 2.90$\pm$0.04 & 0 & -0.700 & nan & 76 & - \\
			IRAS19548+1951 & RSSge & 19 57 06.38 & +19 59 43.7 & 6000 & nan & nan & 1.35$\pm$0.04 & 2.85$\pm$0.05 & 0 & nan & nan & 79 & - \\
			IRAS20056+1834 & QY Sge  & 20 07 54.8 & +18 42 57 & 5850 & nan & nan & 1.36$\pm$0.04 & 4.43$\pm$0.07 & -0.400 & 1.200 & 1500 & 829 & - \\
		\end{tabular}
	\end{center}
	\caption{Cat. 0}
\end{table}


==> Fig/TableCat1.tex <==
\begin{table}
	\begin{center}
		\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
			IRAS & Name & RA & DEC & T$_\mathrm{eff}$ (K) & P$_\mathrm{orb}$ (days) & $e$ & H-K$_\mathrm{s}$ & W1-W3 & [Fe/H] & [Zn/Ti] & T$_\mathrm{Turn-off}$ & IR Lum. (\%) & Ref. \\
			\hline
			IRAS01427+4633 & BD+46.442 & 01 45 47.03 & +46 49 00.97 & 6250 & 140.820 & 0 & 0.46$\pm$0.07 & 2.83$\pm$0.05 & -0.700 & -0.200 & nan & 27 & - \\
			IRAS04166+5719 & TW Cam  & 04 20 48.1 & +57 26 26 & 4800 & 662.200 & 0.250 & 0.57$\pm$0.05 & 3.01$\pm$0.08 & -0.500 & 0.300 & 1100 & 49 & - \\
			IRAS04440+2605 &  RV Tau  & 04 47 06.8 & +26 10 44 & 4500 & 1198 & nan & 0.61$\pm$0.03 & 3.67$\pm$0.09 & -0.400 & 0.500 & 1100 & 48 & - \\
			IRAS06160-1701 &  UY_CMa  & 06 18 16.367 & -17 02 34.72 & 5500 & nan & nan & 0.59$\pm$0.06 & 3.84$\pm$0.04 & 0 & 1.800 & 1000 & 71 & - \\
			EZ_Gem & EZ Gem & 06 46 04.47 & +13 05 02.4 & 6555 & nan & nan & 0.77$\pm$nan & 2.43$\pm$0.03 & 0 & nan & nan & 11 & - \\
			IRAS06489-0118 & SZ Mon & 06 51 27.8362 & -01 22 16.018 & 4700 & nan & nan & 0.55$\pm$0.07 & 3.05$\pm$0.04 & -0.400 & 0.800 & 1500 & 37 & - \\
			IRAS07008+1050 & HD_52961 & 07 03 39.6314 & +10 46 13.067 & 6000 & 1288.600 & 0.230 & 0.45$\pm$0.04 & 2.13$\pm$0.08 & -4.800 & 3 & 1100 & 15 & - \\
			IRAS07140-2321 & SAO_173329 & 07 16 08.271 & -23 27 01.61 & 7000 & 115.900 & 0 & 0.56$\pm$0.04 & 3.64$\pm$0.04 & -0.800 & -0.100 & nan & 47 & - \\
			IRAS08544-4431 & V390 Vel & 08 56 14.182 & -44 43 10.73 & 7250 & 501.100 & 0.200 & 0.97$\pm$0.25 & 3.14$\pm$0.40 & -0.500 & 0.900 & 1200 & 60 & - \\
			IRAS09060-2807 &  V*BZPyx & 09 08 10.1 & -28 19 10 & 6500 & 372 & nan & 0.99$\pm$0.05 & 2.91$\pm$0.06 & -0.500 & 0.200 & nan & 347 & - \\
			IRAS09144-4933 &  ------  & 09 16 09.1 & -49 46 06 & 5750 & 1762 & 0.300 & 0.71$\pm$0.04 & 3.43$\pm$0.08 & -0.500 & nan & 1400 & 67 & - \\
			IRAS09256-6324 &  IW_Car  & 09 26 53.4 & -63 37 48 & 6700 & 1449 & nan & 0.69$\pm$0.26 & 3.71$\pm$0.20 & -1 & 2.100 & 1100 & 69 & - \\
			IRAS09538-7622 &  GP Cha & 09 53 58.5 & -76 36 53 & 5500 & nan & nan & 0.80$\pm$0.05 & 3.00$\pm$0.05 & -0.500 & 0 & nan & 110 & - \\
			IRAS10158-2844 & HR_4049 & 10 18 07.5903 & -28 59 31.201 & 7500 & 430.600 & 0.300 & 1.00$\pm$0.30 & 2.73$\pm$0.12 & -4.500 & nan & 800 & 18 & - \\
			IRAS11000-6153 & HD_95767 & 11 02 04.314 & -62 09 42.84 & 7600 & 1989 & 0.250 & 0.82$\pm$0.05 & 3.36$\pm$0.10 & 0.100 & nan & nan & 56 & - \\
			IRAS11118-5726 &  GK_Car  & 11 14 01.3 & -57 43 09 & 5500 & nan & nan & 0.49$\pm$0.05 & 4.06$\pm$0.03 & -1.300 & 1.200 & 1000 & 64 & - \\
			IRAS11235-5921 & CN Cen & 11 25 47.87 & -59 37 55.9 & 5000 & nan & nan & 0.43$\pm$0.03 & 3.29$\pm$0.03 & -1 & nan & nan & nan & - \\
			IRAS11385-5517 & HD101584 & 11 40 58.80553 & -55 34 25.8169 & 7000 & nan & nan & 1.12$\pm$0.26 & 3.53$\pm$0.19 & 0 & nan & nan & 174 & - \\
			IRAS12185-4856 &  SX_Cen  & 12 21 12.6 & -49 12 41 & 6000 & 564.300 & 0 & 0.65$\pm$0.04 & 3.46$\pm$0.06 & -1 & 1.500 & 1100 & 45 & - \\
			IRAS12222-4652 & HD_108015 & 12 24 53.501 & -47 09 07.51 & 7000 & 906.300 & 0 & 1.02$\pm$0.05 & 3.93$\pm$0.09 & -0.100 & 0.100 & nan & 109 & - \\
			IRAS13085-6747 & PX Mus & 13 11 57.46 & -68 03 35.3 & 5000 & 770 & nan & 0.46$\pm$0.03 & 2.80$\pm$0.03 & 0 & nan & nan & 11 & - \\
			IRAS13258-8103 &  ------  & 13 31 07.1 & -81 18 30 & 6000 & nan & nan & 1.06$\pm$0.03 & 3.09$\pm$0.04 & 0 & nan & nan & 139 & - \\
			IRAS14524-6838 & EN TrA, HD131356 & 14 57 00.684 & -68 50 22.879 & 6000 & 1488 & 0.320 & 0.63$\pm$0.04 & 3.57$\pm$0.08 & -0.500 & 0.600 & 1300 & 67 & - \\
			IRAS15469-5311 &  ------  & 15 50 44.0 & -53 20 44 & 7500 & 390.200 & 0.080 & 1.06$\pm$0.05 & 3.36$\pm$0.09 & 0 & 1.800 & 1300 & 68 & - \\
			IRAS16230-3410 &  ------  & 16 26 20.29 & -34 17 12.3 & 6250 & 649.800 & 0 & 0.60$\pm$0.05 & 3.95$\pm$0.04 & -0.500 & 1 & 1500 & 42 & - \\
			IRAS17038-4815 &  ------  & 17 07 36.3 & -48 19 08 & 4750 & 1394 & 0.630 & 0.46$\pm$0.04 & 4.25$\pm$0.06 & -1.500 & 0.700 & 1400 & 85 & - \\
			IRAS17111-1819 & HD155720 & 17 14 03.070 & -18 22 39.513 & 4250 & 712 & nan & 0.36$\pm$0.04 & 3.36$\pm$0.05 & -1 & nan & nan & nan & - \\
			IRAS17243-4348 &  LR_Sco  & 17 27 56.1 & -43 50 48 & 6250 & 475 & nan & 0.79$\pm$0.04 & 3.40$\pm$0.07 & 0 & 0.800 & 1400 & 91 & - \\
			IRAS17250-5951 & UY Ara & 17 29 28.9495 & -59 54 02.040 & 5500 & nan & nan & 0.53$\pm$0.03 & 3.55$\pm$0.03 & -1 & 1.400 & 1000 & 63 & - \\
			IRAS17279-1119 & HD 158616, V340 Sgr & 17 30 46.9247 & -11 22 08.283 & 7400 & 363.300 & 0 & 0.69$\pm$0.05 & 2.50$\pm$0.06 & -0.700 & 0 & nan & 13 & - \\
			IRAS17534+2603 & 89 Her & 17 55 25.1889 & +26 02 59.966 & 6500 & 289.100 & 0.290 & 0.61$\pm$0.28 & 3.06$\pm$nan & 0 & 0.600 & 1500 & 42 & - \\
			IRAS17530-3348 &  AI_Sco  & 17 56 18.5 & -33 48 47 & 5000 & 977 & nan & 0.61$\pm$0.04 & 3.10$\pm$0.08 & 0 & 0.300 & 1100 & 63 & - \\
			IRAS18123+0511 &  ------  & 18 14 49.4 & +05 12 55 & 5000 & nan & nan & 0.64$\pm$0.04 & 3.77$\pm$0.07 & 0 & nan & nan & 128 & - \\
			IRAS18548-0552 & BZ Sct & 18 57 33.42 & -05 47 55.7 & 6250 & nan & nan & 0.48$\pm$0.03 & 4.42$\pm$0.03 & -0.800 & 1.300 & 1000 & 42 & - \\
			IRAS19135+3937 & nan & 19 15 12.5 & +39 42 51.0 & 6000 & 126.970 & 0.130 & 0.56$\pm$0.03 & 3.16$\pm$0.04 & -0.500 & 0.500 & 1500 & 20 & - \\
			IRAS19157-0247 & V1801 Aql & 19 18 22.5 & -02 42 09 & 7750 & 119.800 & 0.340 & 1.07$\pm$0.04 & 3.61$\pm$0.07 & 0 & nan & 1500 & 73 & - \\
			IRAS19199+3950 & HP Lyr & 19 21 39.07 & +39 56 08.1 & 6300 & 1818 & 0.200 & 0.64$\pm$0.03 & 3.77$\pm$0.05 & -1 & 2.600 & 1300 & 29 & - \\
			IRAS19370+0829 & EZ Aql & 19 39 29.676 & +08 36 27.94 & 5500 & nan & nan & 0.62$\pm$0.03 & 3.02$\pm$0.03 & -1 & nan & nan & 36 & - \\
			IRAS19410+3733 & HD186438 & 19 42 52.92 & +37 40 41.46 & 6500 & nan & nan & 0.33$\pm$0.02 & 3.12$\pm$0.06 & -1 & nan & nan & 27 & - \\
			IRAS19587+3928 & GK Cyg & 20 00 34.48 & +39 36 35.7 & 5250 & nan & nan & 0.33$\pm$0.03 & 2.96$\pm$0.03 & 0 & nan & nan & 46 & - \\
			IRAS19580-3038 & V1711 Sgr & 20 01 07.9832 & -30 30 38.877 & 5000 & nan & nan & 0.49$\pm$0.06 & 3.44$\pm$0.03 & -1.200 & nan & nan & 38 & - \\
			IRAS20094+3721 & nan & 20 11 16.814 & +37 30 52.04 & 5750 & nan & nan & 0.37$\pm$0.03 & 3.53$\pm$0.04 & 0 & nan & nan & 18 & - \\
			IRAS20117+1634 &  R_Sge  & 20 14 03.8 & +16 43 35 & 5750 & nan & nan & 0.67$\pm$0.03 & 3.27$\pm$0.10 & -0.500 & 1.100 & 1200 & 97 & - \\
			IRAS20131+2554 & V*EF_Vul & 20 15 18.60 & +26 03 37.94 & 4250 & nan & nan & 0.38$\pm$0.06 & 3.35$\pm$0.03 & 0 & nan & nan & nan & - \\
			IRAS20343+2625 & V Vul  & 20 36 31.8 & +26 36 17 & 5250 & nan & nan & 0.57$\pm$0.06 & 2.75$\pm$0.08 & 0 & -0.100 & nan & 36 & - \\
			IRAS20401+2550 & HD 340949 & 20 42 20.668 & +26 01 22.36 & 5000 & nan & nan & 0.34$\pm$0.03 & 2.44$\pm$0.11 & 0 & nan & nan & 15 & - \\
			IRAS22223+5556 & BT Lac & 22 24 13.77 & +56 11 33.3 & 5250 & 650 & nan & 0.64$\pm$0.04 & 3.33$\pm$0.03 & 0 & 0.500 & 1400 & 36 & - \\
			IRAS22327-1731 & HD_213985 & 22 35 27.5259 & +39 56 08.1 & 8250 & 259.600 & 0.210 & 0.89$\pm$0.05 & 3.18$\pm$0.07 & -1 & nan & 1000 & 26 & - \\
		\end{tabular}
	\end{center}
	\caption{Cat. 1}
\end{table}


==> Fig/TableCat2.tex <==
\begin{table}
	\begin{center}
		\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
			IRAS & Name & RA & DEC & T$_\mathrm{eff}$ (K) & P$_\mathrm{orb}$ (days) & $e$ & H-K$_\mathrm{s}$ & W1-W3 & [Fe/H] & [Zn/Ti] & T$_\mathrm{Turn-off}$ & IR Lum. (\%) & Ref. \\
			\hline
			IRAS06034+1354 &  DY_Ori  & 06 06 14.91 & +13 54 19.1 & 6000 & 1248 & 0.220 & 0.23$\pm$0.02 & 5.10$\pm$0.05 & -2 & 2.100 & 1000 & 53 & - \\
			IRAS06472-3713 &  ST_Pup  & 06 48 56.4131 & -37 16 33.332 & 5750 & 417.400 & 0 & 0.16$\pm$0.06 & 5.30$\pm$0.03 & -1.500 & 2.100 & 800 & 75 & - \\
			IRAS11472-0800 &  AF Crt & 11 49 48.5 & -08 17 21 & 5750 & nan & nan & 0.41$\pm$0.03 & 6.40$\pm$0.02 & -2.500 & 3.400 & 1000 & 59 & - \\
			IRAS12067-4508 &  RU_Cen  & 12 09 23.7 & -45 25 35 & 6000 & 1489 & 0.620 & 0.24$\pm$0.05 & 4.95$\pm$0.05 & -2 & 1 & 800 & 39 & - \\
			IRAS17233-4330 & V1504 Sco & 17 26 57.5 & -43 33 13 & 6250 & 735 & nan & 1.18$\pm$0.04 & 5.19$\pm$0.03 & -1 & 1.400 & 1000 & 509 & - \\
			IRAS18281+2149 &  AC_Her  & 18 30 16.2 & +21 52 00 & 5500 & 1188.900 & 0 & 0.20$\pm$0.02 & 5.41$\pm$0.08 & -1.500 & 1 & 1200 & 37 & - \\
			IRAS18564-0814 &  AD_Aql  & 18 59 08.1 & -08 10 14 & 6300 & nan & nan & 0.08$\pm$0.03 & 5.07$\pm$0.03 & -2.100 & 2.500 & 1000 & 35 & - \\
		\end{tabular}
	\end{center}
	\caption{Cat. 2}
\end{table}


==> Fig/TableCat3.tex <==
\begin{table}
	\begin{center}
		\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
			IRAS & Name & RA & DEC & T$_\mathrm{eff}$ (K) & P$_\mathrm{orb}$ (days) & $e$ & H-K$_\mathrm{s}$ & W1-W3 & [Fe/H] & [Zn/Ti] & T$_\mathrm{Turn-off}$ & IR Lum. (\%) & Ref. \\
			\hline
			IRAS05208-2035 &  -------  & 05 22 59.423 & -20 32 53.03 & 4000 & 234.380 & 0 & 0.25$\pm$0.05 & 4.38$\pm$0.05 & 0 & nan & nan & 44 & - \\
			IRAS06072+0953 &  CT_Ori  & 06 09 57.9906 & +09 52 31.869 & 5500 & nan & nan & 0.26$\pm$0.05 & 4.18$\pm$0.05 & -2 & 1.900 & 1200 & 56 & - \\
			IRAS06165+3158 & nan & 06 19 50.625 & +31 56 58.16 & 6555 & 262.600 & 0 & 0.08$\pm$0.03 & 3.85$\pm$0.04 & 0 & 0 & nan & 12 & - \\
			IRAS06452-3456 & nan & 06 47 00.5 & -34 59 53 & 6000 & 215.400 & 0 & 0.29$\pm$0.04 & 2.70$\pm$0.06 & 0 & nan & nan & nan & - \\
			IRAS07284-0940 &  U_Mon  & 07 30 47.5 & -09 46 37 & 5000 & 2550 & 0.250 & 0.18$\pm$0.32 & 4.04$\pm$0.32 & -0.800 & 0 & nan & 57 & - \\
			IRAS07331+0021 & AI CMi & 07 35 41.15 & +00 14 58.00 & 6000 & nan & nan & 0.28$\pm$0.03 & 3.80$\pm$0.09 & 0 & nan & nan & 18 & - \\
			IRAS16278-5526 & GZ Nor & 16 31 53.2 & -55 33 08 & 4750 & nan & nan & 0.21$\pm$0.03 & 3.56$\pm$0.03 & -2 & 0.800 & 800 & 20 & - \\
			IRAS19163+2745 & EP Lyr  & 19 18 19.5 & +27 51 03.2 & 7000 & 1151 & 0.390 & 0.02$\pm$0.04 & 2.71$\pm$0.03 & -1.500 & 1.300 & 800 & 3 & - \\
			IRAS21216+1803 & AU Peg & 21 24 00.2439 & +18 16 43.778 & 5750 & 53 & nan & 0.26$\pm$0.03 & 3.08$\pm$0.05 & -0.200 & nan & nan & 15 & - \\
			IRAS22251+5406 & nan & 22 27 05.12 & +54 21 29.16 & 6125 & nan & nan & 0.10$\pm$0.05 & 3.76$\pm$0.04 & 0 & nan & nan & 13 & - \\
		\end{tabular}
	\end{center}
	\caption{Cat. 3}
\end{table}


==> Fig/TableCat4.tex <==
\begin{table}
	\begin{center}
		\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
			IRAS & Name & RA & DEC & T$_\mathrm{eff}$ (K) & P$_\mathrm{orb}$ (days) & $e$ & H-K$_\mathrm{s}$ & W1-W3 & [Fe/H] & [Zn/Ti] & T$_\mathrm{Turn-off}$ & IR Lum. (\%) & Ref. \\
			\hline
			IRAS06054+2237 & SS Gem & 06 08 35.1084 & +22 37 01.937 & 5400 & nan & nan & 0.12$\pm$0.04 & 0.83$\pm$0.05 & -1 & 2 & 1100 & 2 & - \\
			IRAS06338+5333 & HD46703 & 06 37 52.42 & +53 31 01.957 & 6250 & 597.400 & 0.300 & 0.05$\pm$0.02 & 2.25$\pm$0.03 & -1.500 & 0.900 & 800 & 2 & - \\
			F15240+1452 & HD137569 & 15 26 20.81 & +14 41 36.33 & 12000 & 530 & nan & 0.04$\pm$0.02 & 0.17$\pm$0.03 & -3 & nan & nan & nan & - \\
			CC_Lyr & CC Lyr & 18 33 57.4147 & +31 38 24.181 & 6250 & nan & nan & 0.17$\pm$0.03 & 1.87$\pm$0.03 & -3.500 & nan & 1000 & 3 & - \\
			IRAS18448-0545 & R_Sct & 18 47 28.95 & -05 42 18.54 & 4500 & nan & nan & 0.16$\pm$0.37 & 1.00$\pm$0.31 & -0.500 & nan & nan & 6 & - \\
			IRAS19573+4628 & nan & 19 58 52.4 & +46 36 32. & 5500 & nan & nan & 0.08$\pm$0.37 & 1.00$\pm$0.14 & 0 & nan & nan & 8 & - \\
			IRAS20160+2734 & AU Vul & 20 18 05.886 & +27 44 03.69 & 6000 & nan & nan & 0.20$\pm$0.05 & 1.09$\pm$0.06 & 0 & nan & nan & 5 & - \\
			BD+39_4926 & BD+394926 & 22 46 11.2273 & +40 06 26.294 & 7500 & 871.700 & nan & 0.02$\pm$0.02 & 0.64$\pm$0.03 & -2.900 & 2 & 1000 & 1 & - \\
		\end{tabular}
	\end{center}
	\caption{Cat. 4}
\end{table}


==> FinalTable_Paper.tex <==
%\begin{footnotesize}

\setcounter{LTchunksize}{10}
\begin{longtable}{llllc}
\caption{Full list of Galactic sources. We list the IRAS name, alternative identifications, coordinates and the reference to the paper which was used to assemble this list.}\\
%\centering
\label{Table:list}
%\begin{tabular}
\hline
IRAS&Name&a(2000)&d(2000)&Reference selection \\ \hline
\endfirsthead
\caption{continued.}\\
IRAS&Name&a(2000)&d(2000)&Reference selection \\ \hline
IRAS01427+4633 &BD+46.442&01 45 47.03  & +46 49 00.97&h\\
IRAS04166+5719&TW\,Cam &04 20 48.1& +57 26 26&a\\
IRAS04440+2605& RV\,Tau &04 47 06.8& +26 10 44&a\\
IRAS05208-2035&  &05 22 59.423& $-$20 32 53.03&a\\
IRAS06034+1354& DY\,Ori &06 06 14.91& +13 54 19.1&a\\
IRAS06054+2237&SS\,Gem&06 08 35.1084& +22 37 01.937&b\\
IRAS06072+0953& CT\,Ori &06 09 57.9906& +09 52 31.869&a\\
IRAS06108+2743&SU\,Gem &06 14 00.0227& +27 42 12.218&a\\
IRAS06160-1701& UY\,CMa &06 18 16.367& $-$17 02 34.72&a\\
IRAS06165+3158&&06 19 50.625& +31 56 58.16&b\\
IRAS06176-1036& HD\,44179 &06 19 58.2160& $-$10 38 14.691&a\\
IRAS06338+5333&HD\,46703 &06 37 52.42& +53 31 01.957&a\\
&EZ Gem&06 46 04.47& +13 05 02.4 &b\\
IRAS06452-3456&&06 47 00.5& $-$34 59 53&j\\
IRAS06472-3713& ST\,Pup &06 48 56.4131& $-$37 16 33.332&a\\
IRAS06489-0118&SZ\,Mon&06 51 27.8362& $-$01 22 16.018&b\\
IRAS07008+1050& HD\,52961 &07 03 39.6314& +10 46 13.067&a\\
IRAS07140-2321& SAO\,173329 &07 16 08.271& $-$23 27 01.61&a\\
IRAS07284-0940& U\,Mon &07 30 47.5& $-$09 46 37&a\\
IRAS07331+0021 &AI\,CMi&07 35 41.15& +00 14 58.00&e\\
IRAS08011-3627& AR\,Pup &08 03 01.1& $-$36 35 47&a\\
IRAS08544-4431&V390\,Vel&08 56 14.182& $-$44 43 10.73&a\\
IRAS09060-2807& V*BZPyx&09 08 10.1& $-$28 19 10&a\\
IRAS09144-4933&  &09 16 09.1& $-$49 46 06&a\\
IRAS09256-6324& IW\,Car &09 26 53.4& $-$63 37 48&a\\
IRAS09538-7622& GP\,Cha&09 53 58.5& $-$76 36 53&a\\
IRAS10158-2844& HR\,4049 &10 18 07.5903& $-$28 59 31.201&a\\
IRAS10456-5712& HD\,93662 &10 47 38.3965& $-$57 28 02.679&a\\
IRAS11000-6153& HD\,95767 &11 02 04.314& $-$62 09 42.84&a\\
IRAS11118-5726& GK\,Car &11 14 01.3& $-$57 43 09&a\\
IRAS11235-5921&CN\,Cen&11 25 47.87& $-$59 37 55.9&b\\
IRAS11385-5517&HD\,101584&11 40 58.80553& $-$55 34 25.8169&k\\
IRAS11472-0800& AF\,Crt &11 49 48.5& $-$08 17 21&a\\
IRAS12067-4508& RU\,Cen &12 09 23.7& $-$45 25 35&a\\
IRAS12185-4856& SX\,Cen &12 21 12.6& $-$49 12 41&a\\
IRAS12222-4652& HD\,108015 &12 24 53.501& $-$47 09 07.51&a\\
IRAS13085-6747&PX\,Mus&13 11 57.46& $-$68 03 35.3&b\\
IRAS13110-5425&HD\,114855&13 14 08.26&$-$54 41 34.63&g\\
IRAS13258-8103&  &13 31 07.1& $-$81 18 30&a\\
IRAS14524-6838 &EN\,TrA, HD131356&14 57 00.684& $-$68 50 22.879&a\\
IRASF15240+1452&HD\,137569&15 26 20.81&+14 41 36.33&d\\
IRAS15469-5311&  &15 50 44.0& $-$53 20 44&a\\
IRAS15556-5444&  &15 59 32.1& $-$54 53 18&a\\
IRAS16230-3410&  &16 26 20.29& $-$34 17 12.3&a\\
IRAS16278-5526&GZ\,Nor&16 31 53.2& -55 33 08&c\\
IRAS16399-6247&CPD$-$62 5428&16 44 35.37&-62 53 26.00&f\\
IRAS17038-4815&  &17 07 36.3& $-$48 19 08&a\\
IRAS17111-1819&HD\,155720&17 14 03.070&$-$18 22 39.513&n\\
IRAS17233-4330& V1504 Sco&17 26 57.5& $-$43 33 13&a\\
IRAS17243-4348& LR\,Sco &17 27 56.1& $-$43 50 48&a\\
IRAS17250-5951&UY\,Ara&17 29 28.9495& $-$59 54 02.040&b\\
IRAS17279-1119&HD\,158616, V340 Sgr&17 30 46.9247& $-$11 22 08.283&b\\
IRAS17534+2603&89\,Her &17 55 25.1889& +26 02 59.966&a\\
IRAS17530-3348& AI\,Sco &17 56 18.5& $-$33 48 47&a\\
IRAS18123+0511&  &18 14 49.4& +05 12 55&a\\
IRAS18158-3445&  &18 19 13.6& $-$34 44 32&a\\
&AZ\,Sgr&18 24 11.11&-30 25 48.26&i \\
IRAS18281+2149& AC\,Her &18 30 16.2& +21 52 00&a\\
&CC\,Lyr&18 33 57.4147& +31 38 24.181&f\\
IRAS18448-0545 & R\,Sct & 18 47 28.95 & $-$05 42 18.54& b\\
IRAS18548-0552&BZ\,Sct&18 57 33.42& $-$05 47 55.7 &l\\
IRAS18564-0814& AD\,Aql &18 59 08.1& $-$08 10 14&a\\
IRAS19125+0343&BD+03$^{\circ}$3950&19 15 01.1809& +03 48 42.703&a\\
IRAS19135+3937&&19 15 12.5& +39 42 51.0&m\\
IRAS19163+2745&EP\,Lyr &19 18 19.5& +27 51 03.2&a\\
IRAS19157-0247& V1801\,Aql&19 18 22.5& $-$02 42 09&a\\
IRAS19199+3950&HP\,Lyr&19 21 39.07& +39 56 08.1&j\\
IRAS19370+0829&EZ\,Aql&19 39 29.676& +08 36 27.94&b\\
IRAS19410+3733&HD\,186438&19 42 52.92& +37 40 41.46&b\\
IRAS19472+4254&DF\,Cyg&19 48 53.9423& +43 02 14.529&b\\
IRAS19548+1951&RS\,Sge&19 57 06.38& +19 59 43.7&b\\
IRAS19573+4628&&19 58 52.4& +46 36 32.&n\\
IRAS19587+3928&GK\,Cyg&20 00 34.48& +39 36 35.7&b\\
IRAS19580-3038&V1711\,Sgr&20 01 07.9832& $-$30 30 38.877&b\\
IRAS20056+1834&QY\,Sge &20 07 54.8& +18 42 57&a\\
IRAS20094+3721&&20 11 16.814& +37 30 52.04&n\\
IRAS20117+1634& R\,Sge &20 14 03.8& +16 43 35&a\\
IRAS20131+2554&V*EF\,Vul&20 15 18.60&+26 03 37.94&n\\
IRAS20160+2734&AU\,Vul&20 18 05.886& +27 44 03.69&n\\
IRAS20343+2625&V\,Vul &20 36 31.8& +26 36 17&a\\
IRAS20401+2550&HD\,340949&20 42 20.668& +26 01 22.36&n\\
IRAS21216+1803&AU\,Peg&21 24 00.2439& +18 16 43.778&n\\
IRAS22223+5556&BT\,Lac&22 24 13.77& +56 11 33.3&b\\
IRAS22251+5406&&22 27 05.12& +54 21 29.16&n\\
IRAS22327-1731&HD\,213985 &22 35 27.5259&-17 15 26.88 &a\\
 &BD+39$^{\circ}$4926&22 46 11.2273& +40 06 26.294&a\\ \hline
 %\end{tabular}
%\begin{flushleft}
\footnote{(a): \cite{DeRuyter2006}; (b) \cite{Gezer2015}; (c) \cite{Gezer2019}; (d) \cite{Giridhar2005a}; (e) \cite{Klochkova1996}; (f) \cite{Maas2007}; (g) \cite{Giridhar2010}; (h) \cite{Gorlova2012}; (i) \cite{Roa2014}; (j) \cite{Oomen2018}; (k) \cite{Olofsson2015}; (l) \cite{Giridhar2005b}; (m) \cite{Gorlova2015}; (n) This work}
%\end{flushleft}
\end{longtable}
%\end{footnotesize}

==> newtable.tex <==
\begin{sidewaystable*}
\centering
\caption{\label{Table:list} Full list of Galactic sources. The whole table is available online.}
\begin{tabular}{l|l|l|l|c|c|c|c|c|c|c|c|c|c}
\hline\hline
IRAS & Name & RA & DEC & T$_\mathrm{eff}$ & P$_\mathrm{orb}$ & $e$ & H-K$_\mathrm{s}$ & W1-W3 & [Fe/H] & [Zn/Ti] & T$_\mathrm{Turn-off}$ & IR Lum. & Ref. \\
 & & & & (K) & (days) & & & & & & (K) & (\%) & \\
\hline
\multicolumn{10}{l}{Category 0}\\
\hline
06108+2743 & SU\,Gem  & 06 14 00.0 & +27 42 12 & 5750 & 690 & \ldots & 1.45$\pm$0.04 & 3.10$\pm$0.08 & -0.7 & 0.5 & 1400 & 792 & a \\
06176-1036 & HD\,44179, & 06 19 58.2 & -10 38 15 & 7500 & 317.6 & 0.27 & 1.44$\pm$0.25 & 4.48$\pm$0.28 & -3.3 & \ldots & 1000 & 1034 & a \\
 & Red Rectangle &&&&&&&&&&&& \\
08011-3627 &  AR\,Pup  & 08 03 01.1 & -36 35 47 & 6000 & 1250 & \ldots & 1.51$\pm$0.05 & 3.66$\pm$0.40 & -1.0 & \ldots & 1200 & 915 & a \\
15556-5444 &  \ldots  & 15 59 32.1 & -54 53 18 & 6000 & \ldots & \ldots & 1.16$\pm$0.04 & 3.94$\pm$0.08 & 0.0 & \ldots & \ldots & 265 & a \\
18158-3445 &  \ldots  & 18 19 13.6 & -34 44 32 & 6500 & \ldots & \ldots & 1.27$\pm$0.04 & 3.19$\pm$0.04 & 0.0 & \ldots & \ldots & 262 & a \\
19125+0343 & BD+03\,3950 & 19 15 01.2 & +03 48 43 & 7750 & 519.7 & 0.24 & 1.29$\pm$0.04 & 3.38$\pm$0.14 & -0.5 & 2.3 & 1400 & 133 & a \\
19472+4254 & DF\,Cyg & 19 48 53.9 & +43 02 15 & 4800 & 784 & \ldots & 1.16$\pm$0.02 & 2.90$\pm$0.04 &0.0& -0.7 & \ldots & 51 & b \\
19548+1951 & RS\,Sge & 19 57 06.4 & +19 59 44 & 6000 & \ldots & \ldots & 1.35$\pm$0.04 & 2.85$\pm$0.05 &0.0& \ldots & \ldots & 308 & b \\
20056+1834 & QY\,Sge  & 20 07 54.8 & +18 42 57 & 5850 & \ldots & \ldots & 1.36$\pm$0.04 & 4.43$\pm$0.07 & -0.4 & 1.2 & 1500 & 574 & a \\
\hline
\multicolumn{10}{l}{Category 1}\\
\hline 
01427+4633 & BD+46.442 & 01 45 47.0 & +46 49 01 & 6250 & 140.82 &0.0& 0.46$\pm$0.07 & 2.83$\pm$0.05 & -0.7 & -0.2 & \ldots & 16 & h \\
04166+5719 & TW Cam  & 04 20 48.1 & +57 26 26 & 4800 & 662.2 & 0.25 & 0.57$\pm$0.05 & 3.01$\pm$0.08 & -0.5 & 0.3 & 1100 & 46 & a \\
04440+2605 &  RV Tau  & 04 47 06.8 & +26 10 44 & 4500 & 1198 & \ldots & 0.61$\pm$0.03 & 3.67$\pm$0.09 & -0.4 & 0.5 & 1100 & 39 & a \\
06160-1701 &  UY\,CMa  & 06 18 16.4 & -17 02 35 & 5500 & \ldots & \ldots & 0.59$\pm$0.06 & 3.84$\pm$0.04 & 0.0 & 1.8 & 1000 & 69 & a \\
\ldots & EZ\,Gem & 06 46 04.5 & +13 05 02 & 6555 & \ldots & \ldots & 0.77 & 2.43$\pm$0.03 & 0.0 & \ldots & \ldots & 53 & b \\
06489-0118 & SZ Mon & 06 51 27.8 & -01 22 16 & 4700 & \ldots & \ldots & 0.55$\pm$0.07 & 3.05$\pm$0.04 & -0.4 & 0.8 & 1500 & 38 & b \\
07008+1050 & HD\,52961 & 07 03 39.6 & +10 46 13 & 6000 & 1288.6 & 0.23 & 0.45$\pm$0.04 & 2.13$\pm$0.08 & -4.8 & 3.0 & 1100 & 16 & a \\
07140-2321 & SAO\,173329 & 07 16 08.3 & -23 27 02 & 7000 & 115.9 &0.0& 0.56$\pm$0.04 & 3.64$\pm$0.04 & -0.8 & -0.1 & \ldots & 33 & a \\
08005-2356 & V510 Pup & 08 00 32.6 & -23 56 15 & 7000 & 2654 & 0.36 & 1.01$\pm$0.04 & 3.66$\pm$0.09 & -1.0 & \ldots & \ldots & 67 & m \\
08544-4431 & V390 Vel & 08 56 14.2 & -44 43 11 & 7250 & 501.1 & 0.2 & 0.97$\pm$0.25 & 3.14$\pm$0.40 & -0.5 & 0.9 & 1200 & 29 & a \\
09060-2807 &  V*BZPyx & 09 08 10.1 & -28 19 10 & 6500 & 372 & \ldots & 0.99$\pm$0.05 & 2.91$\pm$0.06 & -0.5 & 0.2 & \ldots & 74 & a \\
09144-4933 &  \ldots  & 09 16 09.1 & -49 46 06 & 5750 & 1762 & 0.3 & 0.71$\pm$0.04 & 3.43$\pm$0.08 & -0.5 & \ldots & 1400 & 78 & a \\
09256-6324 &  IW\,Car  & 09 26 53.4 & -63 37 48 & 6700 & 1449 & \ldots & 0.69$\pm$0.26 & 3.71$\pm$0.20 & -1.0 & 2.1 & 1100 & 87 & a \\
09538-7622 &  GP\,Cha & 09 53 58.5 & -76 36 53 & 5500 & \ldots & \ldots & 0.80$\pm$0.05 & 3.00$\pm$0.05 & -0.5 & 0.0 & \ldots & 95 & a \\
10158-2844 & HR\,4049 & 10 18 07.6 & -28 59 31 & 7500 & 430.6 & 0.3 & 1.00$\pm$0.30 & 2.73$\pm$0.12 & -4.5 & \ldots & 800 & 26 & a \\
11000-6153 & HD\,95767 & 11 02 04.3 & -62 09 43 & 7600 & 1989 & 0.25 & 0.82$\pm$0.05 & 3.36$\pm$0.10 & 0.1 & \ldots & \ldots & 84 & a \\
11118-5726 &  GK\,Car  & 11 14 01.3 & -57 43 09 & 5500 & \ldots & \ldots & 0.49$\pm$0.05 & 4.06$\pm$0.03 & -1.3 & 1.2 & 1000 & 64 & a \\
11235-5921 & CN\,Cen & 11 25 47.9 & -59 37 56 & 5000 & \ldots & \ldots & 0.43$\pm$0.03 & 3.29$\pm$0.03 & -1.0 & \ldots & \ldots & 45 & b \\
11385-5517 & HD\,101584 & 11 40 58.8 & -55 34 26 & 7000 & \ldots & \ldots & 1.12$\pm$0.26 & 3.53$\pm$0.19 & 0.0 & \ldots & \ldots & 135 & j \\
12185-4856 &  SX\,Cen  & 12 21 12.6 & -49 12 41 & 6000 & 564.3 &0.0& 0.65$\pm$0.04 & 3.46$\pm$0.06 & -1.0 & 1.5 & 1100 & 30 & a \\
12222-4652 & HD\,108015 & 12 24 53.5 & -47 09 08 & 7000 & 906.3 &0.0& 1.02$\pm$0.05 & 3.93$\pm$0.09 & -0.1 & 0.1 & \ldots & 108 & a \\
13085-6747 & PX Mus & 13 11 57.5 & -68 03 35 & 5000 & 770 & \ldots & 0.46$\pm$0.03 & 2.80$\pm$0.03 & 0.0 & \ldots & \ldots & 12 & b \\
13258-8103 &  \ldots  & 13 31 07.1 & -81 18 30 & 6000 & \ldots & \ldots & 1.06$\pm$0.03 & 3.09$\pm$0.04 & 0.0 & \ldots & \ldots & 284 & a \\
14524-6838 & EN TrA, HD131356 & 14 57 00.7 & -68 50 23 & 6000 & 1488 & 0.32 & 0.63$\pm$0.04 & 3.57$\pm$0.08 & -0.5 & 0.6 & 1300 & 78 & a \\
15469-5311 &  \ldots  & 15 50 44.0 & -53 20 44 & 7500 & 390.2 & 0.08 & 1.06$\pm$0.05 & 3.36$\pm$0.09 & 0.0 & 1.8 & 1300 & 95 & a \\
16230-3410 &  \ldots  & 16 26 20.3 & -34 17 12 & 6250 & 649.8 &0.0& 0.60$\pm$0.05 & 3.95$\pm$0.04 & -0.5 & 1.0 & 1500 & 53 & a \\
17038-4815 &  \ldots  & 17 07 36.3 & -48 19 08 & 4750 & 1394 & 0.63 & 0.46$\pm$0.04 & 4.25$\pm$0.06 & -1.5 & 0.7 & 1400 & 91 & a \\
17111-1819 & HD155720 & 17 14 03.1 & -18 22 40 & 4250 & 712 & \ldots & 0.36$\pm$0.04 & 3.36$\pm$0.05 & -1 & \ldots & \ldots & 19 &n\\
\hline
\multicolumn{14}{l}{\tablebib{(a): \citet{DeRuyter2006}; (b) \citet{Gezer2015}; (c) \citet{Gezer2019}; (d) \citet{Giridhar2005a}; (e) \citet{Klochkova1996}; (f) \citet{Maas2007}; (g) \citet{Giridhar2010}; (h) \citet{Gorlova2012}; (i) \citet{Oomen2018}; (j) \citet{Olofsson2015}; (k) \citet{Giridhar2005b}; (l) \citet{Gorlova2015}; (m) \citet{Manick2021};  (n) This work}}
\end{tabular}
\tablefoot{We list the IRAS name, alternative identifications, coordinates and the reference to the paper which was used to assemble this list. A complete table with all the objects characteristics used in the study will be available online.}
%\end{sidewaystable}
\end{sidewaystable*}
% End longtab


%
